Free flexural vibration of functionally graded size-dependent nanoplates

In this paper, the linear free flexural vibration behaviour of functionally graded (FG) size-dependent nanoplates are investigated using the finite element method. The field variables are approximated by non-uniform rational B-splines. The size-dependent FG nanoplate is investigated by using Eringen's differential form of nonlocal elasticity theory. The material properties are assumed to vary only in the thickness direction and the effective properties for FG nanoplate are computed using Mori-Tanaka homogenization scheme. The accuracy of the present formulation is tested considering the problems for which solutions are available. A detailed numerical study is carried out to examine the effect of material gradient index, the characteristic internal length, the plate thickness, the plate aspect ratio and the boundary conditions on the global response of FG nanoplate.

==> validation.tex <==
Consider a plate of uniform thickness, $h$ and with length and width as $a$ and $b$, respectively. In this case, the displacement field is approximated by Lagrange elements (Q4 and Q8) and with NURBS basis functions. The computed frequencies for a square simply supported plate is given in Table~\ref{table:SSisoplate_comp}. It can be seen that the numerical results from the present study are found to be in good agreement with the existing solutions. Table~\ref{table:SSisoplate_comp} gives the results of non-dimensional frequency for first-order nonlocal plate theory for different values of nonlocal parameter, the plate aspect ratio and for various basis functions. Again, it can be seen that the nonlocal theory predicts smaller values of natural frequency than the local theory. 

% nondimensionalized frequencies
\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Comparison of fundamental frequency $\omega h \sqrt{\rho/G}$ for simply supported plate. $^{\dagger\dagger}$\cite{aghababaeireddy2009}, $^\Box$mesh size 40 $\times 40$, $^\ast$mesh size 8 $\times$ 8, $^\sharp$Order of curve = 3, 5 $\times$ 5 control points.} 
\centering
\begin{tabular}{cccllll}
\hline
$a/b$ & $a/h$ & $\mu$ & Ref.$^{\dagger\dagger}$ & \multicolumn{3}{c}{Method} \\
\cline{5-7}
&  &  &  & Q4$^\Box$ & Q8$^\ast$ & NURBS$^\sharp$\\
\hline
\multirow{6}{*}{1} & \multirow{3}{*}{10} & 0 & 0.0930 & 0.0927 & 0.0926 & 0.0929\\
& & 1 & 0.0850 & 0.0847& 0.0846 &0.0849\\
& & 5 & 0.0660 & 0.0657 & 0.0657 &0.0659\\
\cline{3-7}
& \multirow{3}{*}{20} & 0 & 0.0239 & 0.0240 & 0.0238 &0.0239\\
& & 1 & 0.0218 & 0.0219 & 0.0218 &0.0219\\
& & 5 & 0.0169 & 0.0170 & 0.0169 &0.0170\\
\hline
\multirow{6}{*}{2} & \multirow{3}{*}{10} & 0 & 0.0589 & 0.0588 & 0.0587 &0.0590\\
& & 1 & 0.0556 & 0.0554 & 0.0554 &0.0556\\
& & 5 & 0.0463 & 0.4620 & 0.0462 &0.0464\\
\cline{3-7}
& \multirow{3}{*}{20} & 0 & 0.0150 & 0.0150& 0.0150 & 0.0151\\
& & 1 & 0.0141 & 0.0141& 0.0141 &0.0141\\
& & 5 & 0.0118 & 0.0118& 0.0118 & 0.0118\\
\hline
\end{tabular}
\label{table:SSisoplate_comp}
\end{table}

